Us vs. Them: A Dataset of Populist Attitudes, News Bias and Emotions

Computational modelling of political discourse tasks has become an increasingly important area of research in natural language processing. Populist rhetoric has risen across the political sphere in recent years; however, computational approaches to it have been scarce due to its complex nature. In this paper, we present the new $\textit{Us vs. Them}$ dataset, consisting of 6861 Reddit comments annotated for populist attitudes and the first large-scale computational models of this phenomenon. We investigate the relationship between populist mindsets and social groups, as well as a range of emotions typically associated with these. We set a baseline for two tasks related to populist attitudes and present a set of multi-task learning models that leverage and demonstrate the importance of emotion and group identification as auxiliary tasks.

==> Figures/table.tex <==
\begin{table}[h!]
\centering
\setlength{\tabcolsep}{0.25em}
\begin{tabular}{lccc}
\toprule
 & \textbf{STL} & \textbf{Metaphor} & \textbf{Emotion} \\ \midrule
\multicolumn{1}{l}{\textbf{Political Perspective}} \\
- Center                                                            & .874 & .879 & .885 \\
- Left                                                              & .860 & .863 & .871 \\
- Right                                                             & .774 & .784 & .798 \\ \midrule
\textbf{Political Affiliation} \\
- Democrat                                                          & .788 & .806 & .799 \\
- Republican                                                        & .802 & .805 & .800 \\ \midrule
\textbf{Framing} \\
- Economic                                                          & .747 & .759 & .758 \\
- Capacity and Resources                                            & .601 & .604 & .602 \\
- Morality                                                          & .646 & .662 & .648 \\
- Fairness and Equality                                             & .502 & .527 & .511 \\
- Crime and Punishment                                              & .719 & .721 & .717 \\
- Security and Defense                                              & .554 & .577 & .560 \\
- Health and Safety                                                 & .683 & .694 & .684 \\
- Quality of Life                                                   & .572 & .554 & .556 \\
- Cultural Identity                                                 & .690 & .703 & .695 \\
- Public Sentiment                                                  & .670 & .678 & .675 \\
- Political                                                         & .808 & .815 & .812 \\
- Legality, Constitutionality & \multirow{2}{*}{.787} & \multirow{2}{*}{.795} & \multirow{2}{*}{.784} \\
\ \ and Jurisdiction \\
- Policy Prescription  & \multirow{2}{*}{.525} & \multirow{2}{*}{.538} & \multirow{2}{*}{.530} \\
\ \ and Evaluation \\
- External Regulation & \multirow{2}{*}{.695} & \multirow{2}{*}{.675} & \multirow{2}{*}{.681} \\
\ \ and Reputation \\ \bottomrule
\end{tabular}
\caption{Average F1 for each class and task.}
\label{tab:F1}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table}[h!]
% \resizebox{\columnwidth}{!}{\begin{tabular}{lccc}
%  &
%   \multicolumn{1}{l}{\textbf{Single}} &
%   \multicolumn{1}{l}{\textbf{Metaphors}} &
%   \multicolumn{1}{l}{\textbf{Emotions}} \\ \hline
% \textbf{Hyperpartisan Bias} &
%   \multicolumn{1}{l}{\textbf{}} &
%   \multicolumn{1}{l}{\textbf{}} &
%   \multicolumn{1}{l}{\textbf{}} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% Center                                                                                 & 0.874 & 0.879 & 0.885 \\
% Left                                                                                   & 0.860 & 0.863 & 0.871 \\
% \rowcolor[HTML]{EFEFEF} 
% Right                                                                                  & 0.774 & 0.784 & 0.798 \\ \hline
% \textbf{Political Affiliation}                                                         &       &       &       \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% Democrat                                                                               & 0.788 & 0.806 & 0.799 \\
% Republican                                                                             & 0.802 & 0.805 & 0.800 \\ \hline
% \textbf{Primary Frame}                                                                 &       &       &       \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% Economic                                                                      & 0.747 & 0.759 & 0.758 \\
% \begin{tabular}[c]{@{}l@{}}Capacity and\\ Resources\end{tabular}              & 0.601 & 0.604 & 0.602 \\
% \rowcolor[HTML]{EFEFEF} 
% Morality                                                                      & 0.646 & 0.662 & 0.648 \\
% \begin{tabular}[c]{@{}l@{}}Fairness and\\ Equality\end{tabular}               & 0.502 & 0.527 & 0.511 \\
% \rowcolor[HTML]{EFEFEF} 
% \begin{tabular}[c]{@{}l@{}}Legality, \\ Constitutionality, \\ Jurisdiction\end{tabular} &
%   0.787 &
%   0.795 &
%   0.784 \\
% \begin{tabular}[c]{@{}l@{}}Policy Prescription \\ and Evaluation\end{tabular} & 0.525 & 0.538 & 0.530 \\
% \rowcolor[HTML]{EFEFEF} 
% \begin{tabular}[c]{@{}l@{}}Crime and \\ Punishment\end{tabular}               & 0.719 & 0.721 & 0.717 \\
% \begin{tabular}[c]{@{}l@{}}Security and \\ Defense\end{tabular}               & 0.554 & 0.577 & 0.560 \\
% \rowcolor[HTML]{EFEFEF} 
% Health and Safety                                                             & 0.683 & 0.694 & 0.684 \\
% Quality of Life                                                               & 0.572 & 0.554 & 0.556 \\
% \rowcolor[HTML]{EFEFEF} 
% Cultural Identity                                                             & 0.690 & 0.703 & 0.695 \\
% Public Sentiment
% & 0.670 & 0.678 & 0.675 \\
% \rowcolor[HTML]{EFEFEF} 
% Political                                                                      & 0.808 & 0.815 & 0.812 \\
% \begin{tabular}[c]{@{}l@{}}External Regulation \\ and Reputation\end{tabular} & 0.695 & 0.675 & 0.681
% \end{tabular}}
% \caption{Average F1 for each class and task.}
% \label{tab:F1}
% \end{table}
